ParlayANN: Scalable and Deterministic Parallel Graph-Based Approximate Nearest Neighbor Search Algorithms

Approximate nearest-neighbor search (ANNS) algorithms are a key part of the modern deep learning stack due to enabling efficient similarity search over high-dimensional vector space representations (i.e., embeddings) of data. Among various ANNS algorithms, graph-based algorithms are known to achieve the best throughput-recall tradeoffs. Despite the large scale of modern ANNS datasets, existing parallel graph based implementations suffer from significant challenges to scale to large datasets due to heavy use of locks and other sequential bottlenecks, which 1) prevents them from efficiently scaling to a large number of processors, and 2) results in nondeterminism that is undesirable in certain applications. In this paper, we introduce ParlayANN, a library of deterministic and parallel graph-based approximate nearest neighbor search algorithms, along with a set of useful tools for developing such algorithms. In this library, we develop novel parallel implementations for four state-of-the-art graph-based ANNS algorithms that scale to billion-scale datasets. Our algorithms are deterministic and achieve high scalability across a diverse set of challenging datasets. In addition to the new algorithmic ideas, we also conduct a detailed experimental study of our new algorithms as well as two existing non-graph approaches. Our experimental results both validate the effectiveness of our new techniques, and lead to a comprehensive comparison among ANNS algorithms on large scale datasets with a list of interesting findings.

==> abstract.tex <==
\begin{abstract}
Algorithms for approximate nearest-neighbor search (ANNS) have been
the topic of significant recent interest in the research community.
However, evaluations of such algorithms are usually restricted to a small
number of datasets with millions or tens of millions of points,
whereas real-world applications require algorithms that work on the
scale of billions of points.
Furthermore, existing evaluations of ANNS algorithms are typically
heavily focused on measuring and optimizing for queries-per-second
(QPS) at a given accuracy, which can be hardware-dependent and ignores
important metrics such as build time.

In this paper, we propose a set of principled measures for evaluating
ANNS algorithms which refocuses on their scalability to billion-size
datasets. These measures include ability to be efficiently
parallelized, build times, and scaling relationships as dataset size increases.
%
We also expand on the QPS measure with
machine-agnostic measures such as the number of distance computations per query, and
we evaluate ANNS data structures on their accuracy in more demanding
settings required in modern applications, such as evaluating range
queries and running on out-of-distribution data.
%
We optimize four graph-based algorithms for the billion-scale setting,
and in the process provide a general framework for making many
incremental ANNS graph algorithms lock-free.
%
We use our framework to evaluate the aforementioned graph-based ANNS
algorithms as well as two alternative approaches.
\end{abstract}


==> artifact.tex <==
\newpage

\section{Artifact Instructions}

\paragraph{Code Availability} Our repository can be found at the following \url{https://zenodo.org/records/10223558}. The separate repository that we use to run the algorithms and generate plots (which you should install rather than the above) can be found at this \url{https://zenodo.org/records/10223597}. This repo is what you should download and install, and it contains a Docker container for installing our other library.

\subsection{Getting Started}

We use the Big ANN Benchmarks (\url{https://github.com/harsha-simhadri/big-ann-benchmarks/tree/main}) repository to generate our plots. We have uploaded a fork of this repository to Zenodo (same link as above); you can use it to install a branch of our library that was also uploaded using Zenodo.



\paragraph{Installation} The only prerequisite is Python3.10 and Docker. All commands are assumed to be run in the top-level directory unless otherwise stated. You may wish to use a conda environment for python commands.
\begin{enumerate}
	\item Download and unzip the repo
	\item Run \texttt{pip install -r requirements\_py3.10.txt}
	\item Install docker by following instructions: \url{https://docs.docker.com/engine/install/ubuntu/}.
	You should also to follow the post-install steps for running docker in non-root user mode.
	\item Install the necessary Docker images as follows by running \texttt{python3.10 install.py --algorithm parlayann}
	
	\item Create the result folder by calling \texttt{mkdir results} in the top-level directory

\end{enumerate}


\paragraph{Datasets}

The evaluation assumes that datasets are stored in the \texttt{data/} directory inside the main folder. You should use a symbolic link to a directory on an SSD depending on your memory constraints (this is discussed further in the Evaluation section, note that the resulting saved graphs will also be written to this folder). Download a small toy dataset using:

\begin{verbatim}
python3.10 create_dataset.py --dataset random-xs
\end{verbatim}

\paragraph{Toy Evaluation}

Finally, run the algorithms on the toy dataset to confirm that they run as expected. The `run.py` file builds a nearest neighbor graph (as described in Section 3 of our paper) and queries it, recording the results for later analysis. 

\begin{lstlisting}[breaklines]
python3.10 run.py --algorithm ParDiskANN --dataset random-xs --definitions artifact_eval.yaml
python3.10 run.py --algorithm ParHCNNG --dataset random-xs --definitions artifact_eval.yaml
python3.10 run.py --algorithm ParPyNNDescent --dataset random-xs --definitions artifact_eval.yaml
python3.10 run.py --algorithm ParHNSW --dataset random-xs --definitions artifact_eval.yaml
\end{lstlisting}

Now, generate a plot of results:

\begin{verbatim}
python3.10 plot.py --dataset random-xs
\end{verbatim}

The plot can be found in \texttt{results/random-xs.png}.

\subsection{Evaluation}

Our paper presents results specifically on billion-size datasets. It took around 90 hours on an AWS c6i with 128 vCPUs to build all of the graphs, and requires around 1.5 terabytes of main memory. It additionally requires about 2 TB to store all the datasets, and then an additional 10 TB to store all the graph indices. We assume that the reviewer will not have the relevant time or resources for this evaluation. The evaluation for 100 million size took about 16 hours on an AWS c6i with 128 vCPUs to build each graph and requires about 150 GB of main memory as well as 1 TB storage. We assume that the reviewer may possibly be able to do the 100 million scale evaluation, but we also provide instructions to reproduce the results at the 10 million scale in case that is preferred (the memory requirements scale down by exactly a factor of 10 when going from 100 million to 10 million). 

In the next section, we describe how to reproduce the thread scaling results in Figure~\ref{fig:buildparallelism}. Then, we provide scripts for reproducing the results in Figure~\ref{fig:100Mresults} at either the 10 million or 100 million scale.


\subsection{Thread Scaling}

In Figure~\ref{fig:buildparallelism}, we show speedup of build times relative to the original (i.e. not lock-free) algorithm on one thread. Since the artifact does not require the use of other researchers' code, we instead plot build times for our own implementations on the y-axis and number of threads on the x-axis. 

First, download the dataset:

\begin{verbatim}
	python3.10 create_dataset.py --dataset bigann-1M
\end{verbatim}


The next script builds the graph for each algorithm on [1,2,8,16,24,32,48,64,96] threads. If your evaluation machine has fewer threads, you can access the script and comment out the lines corresponding to the thread counts you wish to exclude. Note that if you are monitoring thread usage using e.g. `htop`, some of the steps outside building (e.g. loading the dataset, saving and loading the graph, etc.) may still use all available threads. 

\begin{verbatim}
bash thread_scaling_bigann.sh
\end{verbatim}

After the run concludes, use the following commands to generate the plot:

\begin{lstlisting}[breaklines]
python3.10 plot.py --dataset bigann-1M -x threads -y build --out results/threadscale_bigann1M -Y log
\end{lstlisting}

You should find the plot in the `results` folder. It should be titled  \texttt{threadscale\_bigann1M.png}.

\subsection{Ten Million Scale QPS/Recall Plots (Figure~\ref{fig:100Mresults})}

First, download the datasets: 
\begin{lstlisting}[breaklines]
python3.10 create_dataset.py --dataset bigann-10M 
python3.10 create_dataset.py --dataset msspacev-10M 
python3.10 create_dataset.py --dataset text2image-10M
\end{lstlisting}

The download of a file occasionally fails due to connectivity and needs to be repeated. Running the download multiple times will not download duplicates of the datasets, so just rerun the same command if you get any error messages.

Next, run each algorithm using the following script:
\begin{verbatim}
bash run_10M_builds.sh
\end{verbatim}

After the run concludes, use the following commands to generate plots:

\begin{verbatim}
bash create_10M_plots.sh
\end{verbatim}

Next, navigate to the `results/` folder. It should have generated three new QPS/recall plots, one for each dataset. 

\subsection{Hundred Million Scale QPS/Recall Plots (Figure~\ref{fig:100Mresults})}

The explanation for these instructions is exactly analogous to the instructions for 10M size datasets:

\begin{lstlisting}[breaklines]
python3.10 create_dataset.py --dataset bigann-100M
python3.10 create_dataset.py --dataset msspacev-100M
python3.10 create_dataset.py --dataset text2image-100M
bash run_100M_builds.sh
bash create_100M_plots.sh
\end{lstlisting}





